Stock2Vec: A Hybrid Deep Learning Framework for Stock Market Prediction with Representation Learning and Temporal Convolutional Network

We have proposed to develop a global hybrid deep learning framework to predict the daily prices in the stock market. With representation learning, we derived an embedding called Stock2Vec, which gives us insight for the relationship among different stocks, while the temporal convolutional layers are used for automatically capturing effective temporal patterns both within and across series. Evaluated on S&P 500, our hybrid framework integrates both advantages and achieves better performance on the stock price prediction task than several popular benchmarked models.

==> stock/tabs/MetricsSector.tex <==
\begin{table}[]
    \caption{Sector level performance comparison}
    \centering
    \label{tab:sector_level}
\resizebox{.8\textwidth}{!}{%
    \begin{tabular}{|cc|c|c|c|c|c|} \hline
        & & Random Forest & Stage-1 &  Stage-2 w. CNN &  Stage-2 w. CS & Full Stage-2 \\ \hline \hline
    % \multirow{3}{*}{AAPL (Apple)} & RMSE & & & & & \\
    Basic Industry & RMSE & 1.370 & & & & \\
                      & MAE & 1.012 & & & & \\
                      & MAPE & 2.214 &&&&\\ \hline 
    Capital Goods & RMSE & 1.277 & & & & \\
                      & MAE & 0.967 & & & & \\
                      & MAPE & 5.077 &&&&\\ \hline 
    Consumer Durables & RMSE & 1.297 & & & & \\
                      & MAE & 0.972 & & & & \\
                      & MAPE & 3.614 &&&&\\ \hline 
    Consumer Non-Durables & RMSE & 1.829 & & & & \\
                      & MAE & 1.242 & & & & \\
                      & MAPE & 4.994 &&&&\\ \hline 
    Consumer Services & RMSE & 1.875 & & & & \\
                      & MAE & 1.200 & & & & \\
                      & MAPE & 4.789 &&&&\\ \hline 
    Energy & RMSE & 1.893 & & & & \\
                      & MAE & 1.362 & & & & \\
                      & MAPE & 2.499 &&&&\\ \hline 
    Finance & RMSE & 1.290 & & & & \\
                      & MAE & 0.933 & & & & \\
                      & MAPE & 5.002 &&&&\\ \hline 
    Healthcare & RMSE & 1.659 & & & & \\
                      & MAE & 1.174 & & & & \\
                      & MAPE & 7.344 &&&&\\ \hline 
    Miscellaneous & RMSE & 1.601 & & & & \\
                      & MAE & 1.230 & & & & \\
                      & MAPE & 5.012 &&&&\\ \hline 
    Public Utilities & RMSE & 1.112 & & & & \\
                      & MAE & 0.836 & & & & \\
                      & MAPE & 4.031&&&&\\ \hline 
    Technology & RMSE & 2.075 & & & & \\
                      & MAE & 1.430 & & & & \\
                      & MAPE & 4.063 &&&&\\ \hline 
    Transportation & RMSE & 1.533 & & & & \\
                      & MAE & 0.977 & & & & \\
                      & MAPE & 2.309 &&&&\\ \hline 
    \end{tabular}
}
\end{table}
